Approximations to the Fisher Information Metric of Deep Generative Models for Out-Of-Distribution Detection

Likelihood-based deep generative models such as score-based diffusion models and variational autoencoders are state-of-the-art machine learning models approximating high-dimensional distributions of data such as images, text, or audio. One of many downstream tasks they can be naturally applied to is out-of-distribution (OOD) detection. However, seminal work by Nalisnick et al. which we reproduce showed that deep generative models consistently infer higher log-likelihoods for OOD data than data they were trained on, marking an open problem. In this work, we analyse using the gradient of a data point with respect to the parameters of the deep generative model for OOD detection, based on the simple intuition that OOD data should have larger gradient norms than training data. We formalise measuring the size of the gradient as approximating the Fisher information metric. We show that the Fisher information matrix (FIM) has large absolute diagonal values, motivating the use of chi-square distributed, layer-wise gradient norms as features. We combine these features to make a simple, model-agnostic and hyperparameter-free method for OOD detection which estimates the joint density of the layer-wise gradient norms for a given data point. We find that these layer-wise gradient norms are weakly correlated, rendering their combined usage informative, and prove that the layer-wise gradient norms satisfy the principle of (data representation) invariance. Our empirical results indicate that this method outperforms the Typicality test for most deep generative models and image dataset pairings.

==> 1_Theory.tex <==

\section{Fisher Information Test Approximation}
\label{sec:Theory}

We wish to utilise a statistic which separates a trained model and the data from which it was trained. 
In such a case, we could view the model as fixed in this statistic, and the evaluation of this statistic against given data as our test hypothesis. 
We wish for this statistic to be natural in the training of our model which lends it to be adaptable and flexible to several neural network architectures. 
For this reason, we consider the log-likelihood of a given function given by 
\begin{align}
    \Lc(\theta, \nu) := \Eb_{X \sim \nu} L_{\theta}(X) = \int L_{\theta}(x) d \nu(x) ,
\end{align}
where $L_{\theta}:X \mapsto \R$ is the likelihood of a specified model with parameters $\theta$ and $\nu$ is a given data set. 
The mapping $\Lc: \mathcal{P} \times \mathbb{P}(X) \mapsto \R$ takes a given set of parameters and a data-set (or measure) on $X$ and returns a real number. 
As $L_{\theta}$ is a likelihood, for a given data sample $\nu$, the more negative $\Lc(\theta, \nu)$, the more probable the model dictated by $\theta$ is for the measure $\nu$.
Let $\nu_{\text{data}}$ be the training data for a given model and assume that the function $\theta \mapsto \Lc(\theta, \nu_{\text{data}})$ is smooth. 
First order convergence of finding the most likely model parameterised by $\theta^*$ for $\nu_{\text{data}}$ occurs when 
\begin{align}
     \left.  \nabla_{\theta} \Lc(\theta,\nu_{\text{data}}) \right|_{\theta = \theta^*}  = \left.   \Eb_{X \sim \nu_{\text{data}}} \nabla_{\theta} L_{\theta}(X) \right|_{\theta = \theta^*} = 0.
\end{align}
Define the functional $\Lc_{\theta^*}: \mathbb{P}(X) \mapsto \R$ through 
\begin{align}
    \Lc_{\theta^*} (\nu) := \left.   \Eb_{X \sim \nu} \nabla_{\theta} L_{\theta}(X) \right|_{\theta = \theta^*}.
\end{align}
The functional $\Lc_{\theta^*}$ takes as input a data-set (or a measure) $\nu$ and returns a real number. 
For the data for which the model was trained on, we expect that $\Lc_{\theta^*}$ has a root at $\nu_{\text{data}}$. 
For data that the model was not trained on, such as $\nu_{\text{anomalous}}$, we expect that
$\Lc_{\theta^*} ( \nu_{\text{anomalous}} ) \neq 0$, or equivalently 
\begin{align}
    \|\Lc_{\theta^*} ( \nu_{\text{anomalous}} )\|_2^2 \neq 0.
\end{align}
Thus a 
\ff{See Chris' write up: https://www.overleaf.com/project/62fa0544a7793625bb1cda5b}



\begin{enumerate}
    \item first point out fisher test for parameters;
    \item look at the dual problem to test for the data;
    \item write down the test statistic;
    \item approximate this with a diagonally dominent matrix.
\end{enumerate}

What computational evidence we need is anything to show diagonal dominance of some of the normalising flow models. 


==> A10_metric_candidate_algorithm.tex <==
\section{A candidate algorithm for computing the Fisher Information Metric via an inner product trick}

\label{sec: candidate algorithm}

TODO if keep: classifier paper uses the same formula but no "inner product trick" \url{https://proceedings.neurips.cc/paper/2020/hash/d1ff1ec86b62cd5f3903ff19c3a326b2-Abstract.html } for pruning

The FIM is defined by:

\[
    F_\theta = \mathbb{E}_{y \sim p^\theta}( \nabla_\theta l(y) \nabla_\theta l(y)^T )
\]

And the score test is defined by:

\[
    \norm{\nabla_\theta l (x)}_{FIM} = \nabla_\theta l(x) F_\theta^{-1} \nabla_\theta l(x)
\]

We want to compute the score test for the distribution $p^\theta$ defined by our DGM, and have the following tools available to us:

\begin{enumerate}
    \item We may sample $y_i \sim p^\theta$ from our model
    \item We may backpropagate gradients $\nabla_\theta l (t)$ for any $t$ in our data space, and store $\approx 50$ of these gradients in memory
    \item We may take the inner product $\nabla_\theta l(t_1)^T \nabla_\theta l(t_2)$ between any two gradient vectors, but not the outer product as that takes too much memory.
\end{enumerate}

We are thus motivated to only ever use the FIM implicitly using an ``inner product trick"

\subsection{Monte-Carlo estimate}

Sample $y_1 \dots y_N$ (for $N \approx 50$) samples from our model and to ease notation set:

\[
    S_i = \nabla_\theta l(y_i)
\]

I propose that we use the biased monte carlo estimate for $F_\theta$ given by 

\[
    F_\theta \approx \frac{1}{N+1} (A_0 + S_1 S_1^T + \dots S_N S_N^T)
\]

where $A_0$ is some diagonal prior guess for $F_\theta$, for example we could just pick the identity matrix or we could pick $diag(\sum_i S_i^2)$ (abusing notation slightly). This still doesn't solve our problem per se, as we still can't compute any of the outer products in the above formula or invert the resulting matrix. Luckily, we have the Sherman-Morrison formula, that gives that:

\[
    (A_0 + S_1 S_1^T)^{-1} 
    = 
    A_0^{-1} - \frac{A_0^{-1} S_1 S_1^T A_0^{-1}}{1 + S_1^T A_0^{-1}S_1}
\]

Letting $S_x = \nabla_\theta l(x)$ We hence see that if $N = 1$ we could compute our approximation to $\norm{\nabla_\theta l(x)}$ by computing:

\[
    \norm{\nabla_\theta l(x)}_{FIM}
    =
    S_x^T F_\theta^{-1} S_x
    \approx 
    2 S_x^T (A_0 + S_1 S_1^T)^{-1} S_x
    =
    2 S_x^T A_0^{-1} S_x -  2 \frac{S_x^T A_0^{-1} S_1 S_1^T A_0^{-1} S_x}{1 + S_1^T A_0^{-1}S_1}
\]

which we see can be computed using only inner products and vector-diagonal matrix products. The idea is that if we set:

\[ 
    A_n = A_{n-1} + S_n S_n^T
\]

Then we could apply the Sherman-Morrison formula recursively, and end up with an approximation of the inverse that, as above, can be computed without needing to store any large matrices. 

\[
    A_n^{-1}
    =
    (A_{n-1} + S_n S_n^T)^{-1} 
    = 
    A_{n-1}^{-1} - \frac{A_{n-1}^{-1} S_n S_n^T A_{n-1}^{-1}}{1 + S_n^T A_{n-1}^{-1}S_n}
\]

I haven't found a compact way to write this out, but I think most of the inner product calculations in practise could be done in parrallel, hopefully making it computationally efficient.

